Meta-theorems for Parameterized Streaming Algorithms

The streaming model was introduced to parameterized complexity independently by Fafianie and Kratsch [MFCS14] and by Chitnis, Cormode, Hajiaghayi and Monemizadeh [SODA15]. Subsequently, it was broadened by Chitnis, Cormode, Esfandiari, Hajiaghayi and Monemizadeh [SPAA15] and by Chitnis, Cormode, Esfandiari, Hajiaghayi, McGregor, Monemizadeh and Vorotnikova [SODA16]. Despite its strong motivation, the applicability of the streaming model to central problems in parameterized complexity has remained, for almost a decade, quite limited. Indeed, due to simple $\Omega(n)$-space lower bounds for many of these problems, the $k^{O(1)}\cdot {\rm polylog}(n)$-space requirement in the model is too strict. Thus, we explore {\em semi-streaming} algorithms for parameterized graph problems, and present the first systematic study of this topic. Crucially, we aim to construct succinct representations of the input on which optimal post-processing time complexity can be achieved. - We devise meta-theorems specifically designed for parameterized streaming and demonstrate their applicability by obtaining the first $k^{O(1)}\cdot n\cdot {\rm polylog}(n)$-space streaming algorithms for well-studied problems such as Feedback Vertex Set on Tournaments, Cluster Vertex Deletion, Proper Interval Vertex Deletion and Block Vertex Deletion. In the process, we demonstrate a fundamental connection between semi-streaming algorithms for recognizing graphs in a graph class H and semi-streaming algorithms for the problem of vertex deletion into H. - We present an algorithmic machinery for obtaining streaming algorithms for cut problems and exemplify this by giving the first $k^{O(1)}\cdot n\cdot {\rm polylog}(n)$-space streaming algorithms for Graph Bipartitization, Multiway Cut and Subset Feedback Vertex Set.

==> OurContribution.tex <==
 %!TEX root = Graph Streaming SODA 22.tex

%\newpage
%\section{Our Contributions and Methodology}\label{sec:ourContribution}
%
%\subsection{Our Contributions: The model}\label{sec:modelInOurContributions}
%
%We introduce the notion of {\em fixed-parameter semi-streaming algorithms} (FPSS algorithms), which are $\wtilde{\bigoh}(f(k)\cdot n)$-space streaming algorithms (for some computable function $f$) that are allowed $f(k)n^{\bigoh(1)}$ time at each edge update and also at the end of the stream, i.e., in post-processing. We initiate the study of FPSS algorithms for well-studied parameterized graph problems as the vast majority of these problems cannot be solved efficiently under the existing notion of parameterized streaming algorithms as discussed earlier.
% We also introduce an appropriate notion of (polynomial) kernelization and (polynomial) compression in the semi-streaming model which are essentially algorithms that run in space $\wtilde\bigoh(k^{\bigoh(1)}n)$ and have polynomially bounded time between edge updates and in post-processing. We lift the classic result equating fixed-parameter tractability and kernelization to this setting, showing equivalence between fixed-parameter semi-streaming and semi-streaming kernelization.
%
%%We also introduce appropriate notions of
%
%
%Our algorithmic contribution consists of two general reduction theorems in the turnstile model that give rise to several corollaries giving fixed-parameter semi-streaming algorithms and polynomial semi-streaming kernelizations for graph modification problems, additional results for specific graph cut problems in the turnstile model, some improvements in the case of insertion-only streams, and then complementary lower bounds. Along the way, we develop sparsification methodologies and combinatorial results that could be of independent interest or of use in the design of other parameterized semi-streaming algorithms. Furthermore, our results imply novel algorithms for well-studied graph problems even in the static setting.
%We now summarize these results in more detail.

%\subsection{Our Contributions: Results}\label{sec:resultsInOurContributions}

%In this subsection, we formalize our all our results and discuss the methodologies in the next subsection.
%
%\medskip
%
%\noindent{\bf Covering Bounded Obstructions.} We begin by giving a general reduction theorem that reduces the problem of vertex deletion into a graph class, to one of simply recognizing the graph class.
%We show that, for any choice of a graph class $\cal H$ that is characterized by excluding a finite set of graphs as induced subgraphs,  if one can solve {\probVDH} when $k=0$ (i.e., decide whether a given graph is in $\cH$) with a semi-streaming algorithm, then one can solve {\probVDH} for any fixed $k$ with a semi-streaming algorithm. More precisely, we prove the following theorem.
%
%\begin{restatable}{theorem}{Hcovering}\label{thm:Hcovering}
%%Let $\cH$ be a finite set of graphs such that $\red{\calG_\cH}$
%Let $\cH$ be a family of graphs defined by a finite number of forbidden induced subgraphs such that $\cH$ admits a deterministic/randomized $p$-pass recognition algorithm in the turnstile (resp.~insertion-only) model for some $p\in\mathbb{N}$. Then, the following hold:
%\begin{enumerate}\item
%    %{\sc $\red{\cG_\cH}$-Vertex Deletion}
%    {\probVDH} admits a deterministic/randomized $p$-pass $\wtilde{\bigoh}(k^{\bigoh(1)}\cdot n)$-space streaming algorithm in the turnstile (resp.~insertion-only) model with post-processing time $2^{\bigoh(k)}\cdot n^{\bigoh(1)}$.
%\item There is a $p$-pass $\wtilde{\bigoh}(k^{\bigoh(1)}\cdot n)$-space polynomial semi-streaming compression  in the turnstile (resp.~insertion-only) model for {\probVDH}.
%%{\sc $\red{\cG_\cH}$-Vertex Deletion}.
%\end{enumerate}
%\end{restatable}
%
%In the above statement,  a $p$-pass recognition algorithm for $\cH$ is a $p$-pass $\widetilde{\OO}(n)$-space streaming algorithm with polynomially bounded time between edge updates and in post-processing that, given a graph $G$, correctly concludes whether or not $G\in \cH$. So, if we can recognize whether a given graph belongs to $\cH$, we can also solve {\probVDH}  as well as attain a polynomial compression for it within the same number of passes and using only $\wtilde{\bigoh}(k^{\bigoh(1)}\cdot n)$-space. Notably, {\em the dependency of the running time we attain on $k$ is the best possible under the Exponential Time Hypothesis {\sc (ETH)}}---even for each of the specific {\probVDH} problems that we consider below (and even for the much simpler {\sc Vertex Cover} problem), it is known that there does not exist a $2^{o(k)}n^{\OO(1)}$-time algorithm under ETH even in the static (non-streaming, where all the input is given directly) setting~\cite{CyganFKLMPPS15}.  We show that several well-studied cases of {\probVDH} admit a $1$-pass recognition algorithm (even in the turnstile model), and thereby attain the following corollary.
%
%\begin{restatable}{corollary}{applicationsOfMainHCoveringTheorem}\label{cor:applicationsOfMainHCoveringTheorem}
%	{\sc Feedback Vertex Set on Tournaments}, {\sc Split Vertex Deletion} and  {\sc Threshold Vertex Deletion}  have 1-pass $\wtilde{\bigoh}(k^{\bigoh(1)}\cdot n)$-space (deterministic) streaming algorithms with $2^{\bigoh(k)}n$-time post-processing and $1$-pass $\wtilde{\bigoh}(k^{\bigoh(1)}\cdot n)$-space polynomial semi-streaming compression in the turnstile model.
%%	\ and $\wtilde{\bigoh}(k^{\bigoh(1)}\cdot n)$-space post-processing.
%	Furthermore, {\sc Cluster Vertex Deletion} has a 1-pass $\wtilde{\bigoh}(k^{\bigoh(1)}\cdot n)$-space  randomized streaming algorithm with $\wtilde{\bigoh}(2^{\bigoh(k)}\cdot n)$-time post-processing in the turnstile model.
%%	\todo{Need to state for all our statements whether they are rand or not, and to add ``in the turnstile model'' (currently it is not done).} \todo{Use restate.}
%\end{restatable}
%
%We remark that when we talk about a randomized algorithm in this paper without explicitly mentioning its success probability, we mean that for every $c>0$, the success probability can be made at least $1-1/n^c$.
%Moreover, although a direct invocation of Theorem~\ref{thm:Hcovering} gives an algorithm whose post-processing FPT algorithm has a polynomial dependence on $n$ in general, in the case of the specific problems above, the respective recognition algorithms have linear-time post-processing, which in fact leads to a linear-time FPT algorithm in the post-processing stage.
%
%\suppressed{
%We further adapt our result to the dual class of {\sc $\cR$-Packing} problems. For a class $\cR$ of graphs, this problem takes as input a graph $G$ and an integer $k\in\mathbb{N}_0$, and the objective is to decide whether there exist at least $k$ vertex-disjoint induced subgraphs in $G$ that are each isomorphic to a graph in $\cR$. Specifically, we attain the following result.
%
%\begin{restatable}{theorem}{Hpacking}\label{thm:Hpacking}
%Let $\cH$ be a family of graphs defined by a finite set $\cR$ of forbidden induced subgraphs such that $\cH$ admits a deterministic/randomized $p$-pass recognition algorithm for some $p\in\mathbb{N}$ in the turnstile (resp.~insertion-only) model. Then,   {\sc $\cR$-Packing} admits a deterministic/randomized $p$-pass $\wtilde{\bigoh}(k^{\bigoh(1)}\cdot n)$-space streaming algorithm with post-processing time $2^{\bigoh(k\log k)}\cdot n^{\bigoh(1)}$ in the turnstile (resp.~insertion-only) model.
%\end{restatable}
%
%This yields the following corollary for certain well-studied packing problems in the graph algorithms literature.
%
%\begin{restatable}{corollary}{applicationsOfMainHPackingTheorem}\label{cor:applicationsOfMainHPackingTheorem}
%	{\sc Tournament Triangle Packing}, $\{C_4,C_5,2K_2\}$-{\sc Packing} and  $\{P_4,C_4,2K_2\}$-{\sc Packing} have 1-pass $\wtilde{\bigoh}(k^{\bigoh(1)}\cdot n)$-space (deterministic) streaming algorithms with $\wtilde{\bigoh}(2^{\bigoh(k \log k)}n)$-time post-processing in the turnstile model.
%%	\ and $\wtilde{\bigoh}(k^{\bigoh(1)}\cdot n)$-space post-processing.
%Furthermore,	$P_3$-{\sc Packing} has a 1-pass $\wtilde{\bigoh}(k^{\bigoh(1)}\cdot n)$-space  randomized streaming algorithm with $\wtilde{\bigoh}(2^{\bigoh(k \log k)}\cdot n)$-time post-processing in the turnstile model.
%% that succeeds with probability at least $1-1/n^c$ for any given $c>0$.  \todo{In previous corollary and other results, we did not mention success prob. Either remove here (and clarify that randomized means high success prob), or fix in other places.}
%\end{restatable}
%}
%
%
%\medskip
%\noindent{\bf Covering Unbounded Obstructions.} By strengthening  the requirements in Theorem \ref{thm:Hcovering}, we obtain a similar result even when the set of forbidden induced subgraphs for $\cH$ may be of infinite size. For example, the obstruction set that defines the class of proper interval graphs is infinite since it contains all chordless cycles. More generally, our result holds for any hereditary graph class (i.e., graph class closed under taking induced subraphs).  Here, we require {\em reconstruction} for $\cH$ rather than recognition for $\cH$, which means that for a given graph $G$, we need to determine whether $G\in \cH$ (as in recognition), but in case the answer is positive, we also need to output a {\em succinct representation of $G$}. Recall that by a succinct representation, we mean a data structure that takes $\widetilde{\OO}(n)$ space and supports ``edge queries''---given a pair of vertices $u,v$, it answer whether $\{u,v\}$ is an edge in $G$. In addition to this requirement, we also suppose to be given an algorithm that solves the problem (in $\widetilde{\OO}(n)$ space) in the static setting, which is clearly an easier task than attaining the same result in the streaming setting. Specifically, we prove the following theorem.
%
%\begin{restatable}{theorem}{reductionLemma}\label{lem:reductionLemma}
%Let $\cH$ be a hereditary graph class such that:
%\begin{enumerate}
%\item\label{item:reduction1} $\cH$ admits a $p$-pass deterministic/randomized reconstruction algorithm for some $p\in\mathbb{N}$ in the turnstile (resp.~insertion-only) model, and
%\item\label{item:reduction2} {\probVDH} admits a deterministic/randomized $\widetilde{\OO}(n\cdot g(k))$-space $f(k)\cdot n^{\OO(1)}$-time (static) algorithm where $g$ and $f$ are some computable functions of $k$. % such that $f(k)\geq 2^k$.
%\end{enumerate}
%Then,  {\probVDH} admits a $p$-pass deterministic/randomized $\widetilde{\OO}(n\cdot g(k)\cdot k^{\OO(1)})$-space streaming algorithm with post-processing time $2^k\cdot f(k) \cdot n^{\OO(1)}$  in the turnstile (resp.~insertion-only) model.
%%\todo{Changed from lemma to theorem (change refs accordingly).} \todo{Use restate.}
%\end{restatable}
%
%We further present a version of this theorem that yields kernels. For this, we define the {\sc VC-Annotated} {\probVDH} problem (where {\sc VC} stands for {\sc Vertex Cover}) as a generalization of {\probVDH} where, in addition to $G$ and $k$, the input also contains a collection of pairs of vertices of $G$. Then, we seek a subset of at most $k$ vertices whose deletion from $G$ yields a graph in $\cH$ and which, for every pair of vertices in the input, contains at least one vertex from that pair. Equivalently, we can suppose to be given another graph on the same vertex set, and require our solution to also be a vertex cover for that graph. Specifically, we prove the following theorem.
%
%\begin{restatable}{theorem}{reductionLemmaKernel}\label{lem:reductionLemmaKernel}
%Let $\cH$ be a hereditary graph class such that
%    \begin{enumerate}
%        \item $\cH$ admits a $p$-pass deterministic/randomized reconstruction algorithm for some $p\in\mathbb{N}$  in the turnstile (resp.~insertion-only) model, and
%        \item {\sc VC-Annotated} {\probVDH} admits a deterministic/randomized $\widetilde{\OO}(n\cdot g(k))$-space $n^{\OO(1)}$-time (static) polynomial kernelization algorithm where $g$ is some polynomial function of $k$.
%        \item{\probVDH} is {\NPC}.
%    \end{enumerate}
%    Then, {\probVDH} admits a $p$-pass deterministic/randomized $\widetilde{\OO}(n\cdot g(k)\cdot k^{\OO(1)})$-space polynomial semi-streaming kernelization algorithm
%%    with post-processing time $n^{\OO(1)}$
%    in the turnstile (resp.~insertion-only) model.
%%     that outputs a polynomial kernel of the instance $(G,k)$.
%%     \todo{Changed from lemma to theorem (change refs accordingly).} \todo{Use restate.}
%\end{restatable}
%
%
%
%We remark that having the requirement that the kernel, in the static setting, should exist for {\sc VC-Annotated}
% {\probVDH} rather than for {\probVDH} is not necessarily a stricter requirement since kernels usually (with slight adaptations) work for this more general version.
%
%We demonstrate the applicability of our theorems for the classes of proper intervals graphs and block graphs, where the size of the obstruction set is infinite. For each one of these two problems, we design a reconstruction algorithm, as well as kernel that works in $\widetilde{\OO}(n)$ space in the static setting. Towards the design of these kernels, we also design parameterized algorithms that work in $\widetilde{\OO}(n)$ space, and are adapted to yield also approximation algorithms, in the static setting. We remark that these components may be of independent interest. Overall, this yields the following corollaries.
%
%\begin{corollary}\label{cor:pivdIntro}
%{\sc Proper Interval Vertex Deletion} admits a randomized $\OO(\log^2 n)$-pass $\widetilde{\OO}(k^{\OO(1)}n)$-space streaming algorithm with $2^{\OO(k)}\cdot n^{\OO(1)}$ post-processing time in the turnstile model. Additionally, it admits a randomized $\OO(\log^2 n)$-pass $\widetilde{\OO}(k^{\OO(1)}n)$-space polynomial semi-streaming kernelization in the turnstile model.
%%\todo{$k^{\OO(1)}$ was missing in the space complexity; fixed in the corresponding locations in the technical sections.}
%\end{corollary}
%
%\begin{corollary}\label{cor:blockIntro}
%{\sc Block Vertex Deletion} admits a randomized 1-pass $\widetilde{\OO}(k^{\OO(1)}n)$-space streaming algorithm with $2^{\OO(k)}\cdot n^{\OO(1)}$ post-processing time in the turnstile model. Additionally, it admits a randomized 1-pass $\widetilde{\OO}(k^{\OO(1)}n)$-space polynomial semi-streaming kernelization in the turnstile model.
%\end{corollary}
%
%
%\medskip
%\noindent{\bf Specific Cut Problems.} Before we turn to the insertion-only model and lower bounds, we devise a sampling primitive that we use to deal with additional graph problems, which are not encompassed by the previous theorems. Specifically, we consider the {\sc Odd Cycle Transversal}, {\sc Subset Feedback Vertex Set} and {\sc Multiway Cut} problems. The obstruction set for  {\sc Odd Cycle Transversal} is the set of all odd cycles, and the family of graphs excluding these obstructions includes all bipartite graphs, which cannot be encoded in $\widetilde{\OO}(n)$ space (since there are $2^{\Omega(n^2)}$ different bipartite graphs). As for {\sc Subset Feedback Vertex Set}, the obstruction set is the family of all cycles that contain ``terminals''---the objective of  {\sc Subset Feedback Vertex Set} is to determine whether one can choose at most $k$ vertices that intersect all cycles in the input graph $G$ that pass through at least one designated vertex, called a terminal (the input contains, in addition to $G$ and $k$, a subset of vertices called terminals). Besides the fact that our general reduction theorem does not consider obstructions with terminals, the family of graphs excluding the aforementioned obstruction cannot be encoded in $\widetilde{\OO}(n)$ space since, in particular, this family contains all graphs (without terminals). A similar argument holds in the case of {\sc Multiway Cut} where the obstruction set is the family of all paths that connect pairs of ``terminals''. In this problem, the input is $G$, $k$ and a vertex subset called terminals and the objective is to determine whether a set of at most $k$ vertices intersects every path in $G$ between a pair of terminals.
%Using our sampling primitive along with problem-specific sparsification steps for each of these problems, we derive the following results.
%
%%\begin{restatable}{theorem}{oct}
%%\label{thm:oct}
%%There is a 1-pass $\wtilde{\bigoh}(k^{\bigoh(1)}\cdot n)$-space randomized streaming algorithm for  {\sc OCT} with $\wtilde{\bigoh}(2^{\bigoh(k)}\cdot n)$-time post-processing.
%%\end{restatable} \todo{MZ: I saw you already used restatable, but did not know how to restate it here (before the restatable occurs). So need to restate it there.}
%\begin{restatable}{theorem}{oct}
%\label{thm:oct}
%There is a 1-pass $\wtilde{\bigoh}(k^{\bigoh(1)}\cdot n)$-space randomized streaming algorithm for {\sc OCT} with $\wtilde{\bigoh}(3^{k}k^{\bigoh(1)} n)$-time post-processing.
%\end{restatable}
%
%
%%A semi-streaming algorithm for OCT even with $k=1$ appears to be out of reach of the iterative compression implementation of Chitnis and Cormode~\cite{ChitnisC19} in the streaming setting. In fact, they ask for an $f(k)$-pass $\wtilde{\bigoh}(g(k)\cdot n)$-space algorithm for $k$-OCT. Moreover, there is a $\Omega(n\log n)$-space lower bound for OCT even with $k=0$. Hence, upto $\wtilde{\bigoh}(k^{\bigoh(1)})$ factors in the space bounds, we have essentially given an optimal fixed-parameter semi-streaming algorithm for OCT. \hly{to Intro?}
%
%%We also obtain new algorithms for the
%
%\begin{restatable}{theorem}{subsetFVS}\label{thm:subsetFVS}
%	There is a 1-pass $\wtilde{\bigoh}(k^{\bigoh(1)}\cdot n)$-space randomized streaming algorithm for  {\sc Subset Feedback Vertex Set} with $\wtilde{\bigoh}(2^{\bigoh(k)}\cdot n)$-time post-processing.
%\end{restatable}
%
%
%\begin{restatable}{theorem}{multiwaycut}\label{thm:multiwaycut}
%	There is a 1-pass $\wtilde{\bigoh}(k^{\bigoh(1)}\cdot n)$-space randomized streaming algorithm for  {\sc Multiway Cut} with $\wtilde{\bigoh}(4^kk^{\bigoh(1)}\cdot n)$-time post-processing.
%\end{restatable}
%
%Theorem~\ref{thm:oct} answers an open problem of Chitnis and Cormode~\cite{ChitnisC19}, who ask for an $f(k)$-pass $\wtilde{\bigoh}(g(k)\cdot n)$-space algorithm for OCT and note that even for $k=1$, such an algorithm is not known.
%
%We also remark that the general approach based on the sampling primitive is widely applicable and each specific application essentially boils down to designing, for these problems, (i) problem-specific sparsification subroutines similar to those for the aforementioned specific cut problems and (ii) linear-space (or ideally, linear-time) FPT algorithms for use in post-processing.
%
%\noindent
%{\bf Proof overview for Theorem~\ref{thm:oct}. }At the heart of our algorithms for these cut problems is a sampling primitive based on one of Guha et al.~\cite{GuhaMT15} which they used to estimate vertex connectivity.
%
%The main idea here is to sample roughly $\wtilde\bigoh(k^{\bigoh(1)})$ vertex subsets $V_1,\dots, V_\ell$ of the input graph so that with good probability, for every set $S\subseteq V(G)$ that is disjoint from some forbidden substructure in $G$ (i.e., odd cycles or cycles containing terminals or paths between terminals), the set of sampled vertex sets has the property that the subgraph of $G$ induced by the union of those subsets disjoint from $S$ also contains a forbidden substructure for the problem concerned. This allows us to identify a set of $\wtilde\bigoh(k^{\bigoh(1)}n)$ subgraphs that can always provide a witness when a vertex set is {\em not} a solution for the problem at hand. However, these sampled subgraphs may still be dense and it is far from obvious how one could sparsify them while preserving the aforementioned property. Therefore, for each of the problems we consider in this section, we provide a problem-specific $\wtilde\bigoh(k^{\bigoh(1)}n)$-space sparsification step that allows us to reduce the number of edges we keep from each of the sampled subgraphs to $\bigoh(n)$, while ensuring that non-solutions can still be witnessed by a substructure in the union of the sparsified subgraphs. Finally, we invoke existing linear-time (static) FPT algorithms on the sparsified instance and show that a solution for this reduced instance is also a solution for the original instance.
%
%In the case of OCT, the sparsification step consists of computing a dynamic connectivity sketch for the bipartite double covers (see Section~\ref{sec:cutProblems} for a formal definition) of the sampled subgraphs. For {\sc Subset FVS}, we maintain a dynamic connectivity sketch for the sampled subgraphs along with the edges incident on terminals. For {\sc Multiway Cut}, we simply maintain a dynamic connectivity sketch for the sampled subgraphs. We remark that this final case closely resembles part of the vertex-connectivity approximation algorithm of Guha et al.~\cite{GuhaMT15}.
%
%
%%\medskip
%%\noindent{\bf Results for Insertion-only Streams.} Here, we turn our attention to insertion-only streams and give deterministic FPSS algorithms for several problems.
%%In particular, we revisit Theorem~\ref{thm:Hcovering} and by designing a novel 2-pass recognition algorithm for the class of trivially perfect graphs on insertion-only streams, we obtain the following consequence.
%%
%%
%%
%%\begin{restatable}{corollary}{triviallyPerfectConsequence}\label{cor:triviallyPerfectConsequence}
%%{\sc Trivially Perfect Vertex Deletion} admits a $2$-pass $\widetilde{O}(k^{\OO(1)}\cdot n)$-space deterministic streaming algorithm in the insertion-only model with $\widetilde{O}(2^{\OO(k)}\cdot n)$-time and $\widetilde{O}(k^{\OO(1)}\cdot n)$-space post-processing.
%%\end{restatable}
%%
%%
%%We then revisit the cut problems considered above (details in Section~\ref{sec:cutProblems}) and obtain single pass deterministic FPSS algorithms for {\NPC} edge-deletion variants of these problems. In particular, we consider the {\sc Edge Multiway Cut} problem and {\sc Edge Bipartization} problems. The input to the former is the same as that for {\sc Multiway Cut} and the goal is to determine whether a there is a set of at most $k$ edges that intersects every path connecting a pair of terminals. In the latter, the input is the same as that for {\sc Odd Cycle Transversal} and the goal is to determine whether a set of at most $k$ edges intersects all odd cycles in $G$. We obtain the following results.
%%
%%
%%\begin{restatable}{theorem}{edgeMultiwayCut}\label{thm:edgeMultiwayCut}
%%	There is a 1-pass $\wtilde{\bigoh}(kn)$-space deterministic streaming algorithm for {\sc Edge Multiway Cut} in the insertion-only model
%%	with $\wtilde{\bigoh}(4^{k}k^{\bigoh(1)}n)$-time post-processing.
%%	\end{restatable}
%%
%%\begin{restatable}{theorem}{edgeBipartization}\label{thm:edgeBipartization}
%%	There is a 1-pass $\wtilde{\bigoh}(kn)$-space deterministic streaming algorithm for {\sc Edge Bipartization} in the insertion-only model
%%	with $\wtilde{\bigoh}(3^k k^{\bigoh(1)} n)$-time post-processing.
%%	\end{restatable}
%%
%
%\medskip
%\noindent{\bf Lower Bounds.}
%We prove lower bounds on the space complexity of streaming algorithms for various graph problems. All our lower bounds hold even for randomized algorithms on insertion only streams. We prove that {\sc Split Graph Recognition} by a $1$-pass streaming algorithm takes $\Omega(n)$ space,  almost matching the upper bound of $\wtilde{\bigoh}(n)$ which involves simply maintaining the degree sequence of the graph.
%%For the {\sc Cluster Graph Recognition} problem and
%For the problem of testing whether the input graph has a connected vertex cover of size at most $3$, we show that any $p$-pass streaming algorithm requires at least $\Omega(n/p)$ space. Moreover, these lower bounds almost match the upper bounds for these problems.
%%Indeed, {\sc Cluster Graph Recognition} can be solved by maintaining a connectivity sketch and the degree sequence of the input graph and a streaming algorithm requires only  $\wtilde{\bigoh}(n)$ space to keep the connectivity sketch and the degree sequence of the graph.
%Indeed, if a graph has a connected vertex cover of size $k$, then the number of edges in the graph is at most $kn$. This implies that  a streaming algorithm only requires $\wtilde{\bigoh}(n)$ space to test whether the input graph has a connected vertex cover of constant size.
%
%We also give stronger $\Omega(n \log n)$ and $\Omega(n^2)$ lower bounds for some graph problems. For {\sc Minimum Bisection} (the problem of testing whether the input graph can be partitioned into two equal parts where the  number of crossing edges is at most $k$, where $k$ is also part of the input).
%% and {\sc Long Path} (the problem of testing whether the input graph has a path of given length)
%we give $\Omega(n \log n)$-space lower bounds.
%For the {\sc Chordal Recognition} problem we give an $\Omega(n^2)$ lower bound.
%This should be contrasted with our positive result for recognition of block graphs---in particular, we draw a tractability border between these two classes (recall that the class of block graphs is a subclass of that of chordal graphs).



==> deterministicCutProblems.tex <==


%\subsubsection{Deterministic Algorithms for Edge Versions}
%\newcommand{\inv}{^{-1}}

%\subsection{Min Bisection, Edge Multiway Cut, Subset FES}

%Recall that in the {\sc Edge Multiway Cut} problem, the input is a graph $G$, a set $T\subseteq V(G)$ of terminals and integer $k$ and the goal is to determine whether there is a set of at most $k$ edges whose deletion separates every pair of terminals. As before, we assume the following input model for instances of this problem. For each terminal, when the first edge incident on it is inserted, it is inserted along with a pair of bits that indicate whether (and if so, which of) the endpoints of this edge are terminals.
%
%\edgeMultiwayCut*
%%\begin{theorem}\label{thm:edgeMultiwayCut}
%%	There is a 1-pass $\wtilde{\bigoh}(kn)$-space deterministic streaming algorithm for {\sc Edge Multiway Cut}
%%	with $\wtilde{\bigoh}(4^{k}k^4n)$-time post processing.
%%	\end{theorem}
%
%\begin{proof}
%%In the edge stream we keep $k+1$ ($k+2$ in the case of Subset FES) edge disjoint spanning trees(forests).
%The processing step is as follows. We maintain a set of $k+1$ edge-disjoint spanning forests of the input graph $G$ as follows. Initialize forests $F_1,\dots, F_{k+1}$ with vertex set $V(G)$ and empty edge set.
%   For every edge $e=(u,v)$ that arrives in the stream, we check whether
%   there is an $i\in [k+1]$ such that $u$ and $v$ are not in the same tree of forest $F_i$. If such an $i$ exists, then we find the least such $i$ and add the edge $e$ to the forest $F_i$. Otherwise, we ignore the edge $e$. Let $G'$ be the subgraph of $G$ defined by taking the union of the $k+1$ edge-disjoint spanning forests $F_1,\dots, F_{k+1}$. Clearly, $G'$ has $\bigoh(kn)$ edges and hence can be stored in space $\wtilde\bigoh(kn)$.
%
%
%We now argue that $(G',k)$ is a yes-instance of {\sc Edge Multiway Cut} if and only if $(G,k)$ is a yes-instance of {\sc Edge Multiway Cut}. Since $G'$ is a subgraph of $G$, it is sufficient to argue that if $(G',k)$ is a yes-instance then $(G,k)$ is a yes-instance.
%
%%\begin{description}[style=unboxed,leftmargin=0cm]
%%\item[Min bisection:]  Suppose $(G',k)$ is yes-instance with a solution cut $(A,B)$. We claim that $(A,B)$ is also a solution cut for $(G,k)$. Suppose to the contrary that there is a crossing  edge $(a,b)$ in $E(G)\setminus E(G')$, where $a\in A$ and $b\in B$. As, we did not include $(a,b)$ in our sketch, it must be the case that $a$ and $b$ are connected in all the $k+1$ connectivity sketches, implying that there are $k+1$ edge-disjoint paths in $G'$.  However, since $(A,B)$ is a cut of size at most $k$ in $G'$, we obtain  a contradiction\footnote{We know a conditional randomized XP post processing by invoking this result of Bringmann, but improving any of these constraints  is not entirely clear yet.}. \hly{Need to write about post-processing.}
%Suppose that $(G',k)$ is yes-instance with an inclusionwise minimal solution $S\subseteq E(G')$. We claim that $S$ is also a solution for the instance $(G,k)$. Suppose not. Then, there is an edge $e=(a,b)\in E(G)\setminus E(G')$ that has endpoints in distinct connected components of $G'-S$. By our construction, $e$  can be absent from $G'$ only if there are $k+1$ edge-disjoint $a$-$b$ paths in $G'$. However, since $|S|\leq k$, it follows that  $a$ and $b$ lie in the same connected component of $G'-S$, a contradiction.
%% \end{description}
%
%Given the above the post-processing step for {\sc Edge Multiway Cut} simply invokes the known $4^kk^{\bigoh(1)}(m+n)$-time $k^{\bigoh(1)}(m+n)$-space fixed-parameter algorithm for this problem (see, for example, \cite{CyganFKLMPPS15}).  This completes the proof of the theorem.
%\end{proof}
%
%
%We now move on to the edge version of OCT, i.e., {\sc Edge Bipartization}, where the input is a graph $G$ and integer $k$ and the goal is to determine whether there is a set of at most $k$ edges that intersect every odd cycle in the graph.
%
%%
%\edgeBipartization*
%
%%
%%
%%In the Edge Unique Label Cover (Edge ULC) problem, the input is a simple graph $G$,
%%finite alphabet $\Sigma$, integer $k$ and for every edge $e\in E(G)$ and each of its
%%endpoints $u$, a permutation $\phi_{e,u}$ of $\Sigma$ such that
%%if $e=(u,v)$ then $\phi_{e,u}=\phi_{e,v}^\inv$ and a function $\tau:V\to 2^\Sigma$.
%% The goal is to determine whether there is a set $X\subseteq E(G)$ of size at most $k$ and a function $\Psi:V(G) \to \Sigma$ such that for every $v\in V(G)$, for every $(u,v)\in E(G-X)$, we have $( \Psi(u),\Psi(v))\in \phi_{uv,u}$. We say that $\Psi$ is a {\em feasible labelling} for this instance if for all $(u,v)\in E(G)$, $(\Psi(u),\Psi(v))\in \phi_{uv,u}$.
%%
%%  The standard parameterization for this problem is $|\Sigma|+k$ and Edge Bipartitization is a special case of Edge ULC for $|\Sigma|=2$. We now give the construction for Edge ULC. We use $\ell$ to denote $|\Sigma|$. Moreover, notice that the function $\phi_{e,u}$ can be extended from edges to paths in a natural way by composing the functions on the edges that lie on this path.
%%
%%\smallskip
%%\noindent
%
%\begin{proof}
%Our goal is to keep a subgraph comprising at most $2k+1$ edge-disjoint spanning forests of the input graph plus at most $k+1$ additional edges as follows.
%%The processing step is as follows. We maintain a set of $k+1$ edge-disjoint spanning forests of the input graph $G$ as follows.
% Initialize forests $F_1,\dots, F_{2k+1}$ with vertex set $V(G)$ and empty edge set.
%
%\smallskip
%%\thinblackbox{
%\noindent
%For every inserted edge $e=(u,v)$ of the graph $G$, do:
%%\smallskip
%\begin{enumerate}
%\item  Check if there is an $i\in [2k+1]$ such that $u$ and $v$ are not in the same tree of forest $F_i$.
%\item If such an $i$ exists, then find the least such $i$ and add the edge $e$ to the forest $F_i$.
%%If $u,v$ appear in the same tree in fewer than $2k+1$ edge-disjoint spanning forests, then we locate the least $i$
%\item If $u,v$ appear in the same tree in every $F_i$, then in at least $k+1$ of these forests, the length of the $u$-$v$ path has the same parity.
%%
%%there are $2k+1$ $u$-$v$ paths already present in the sketch, implying that there are $k+1$ $u$-$v$ paths $P_1,\dots, P_{k+1}$ of the same parity.
%%such that for every $i,j\in [k+1]$,  $\phi_{P_{i},u}=\phi_{P_{j},u}$.
%Compute $k+1$ such $u$-$v$ paths $P_1,\dots, P_{k+1}$ of the same parity.  We now we have two subcases.
%
%
%\noindent
%Case (i): For every $i\in [k+1]$, the path $P_i$ is even. Then, mark the edge $e$. If, at any point, the number of marked edges exceeds $k$, then we conclude that the instance is a no-instance and stop storing any more edges after the $(k+1)^{\sf th}$ marked edge. \\
%
%
%\noindent
%Case (ii): Otherwise, we ignore $e$.
%\end{enumerate}
%%}
%
%$G'$ is defined as the subgraph of $G$ induced by the marked edges and the edges in the forests $F_1,\dots, F_{2k+1}$. Notice that $G'$ has $\bigoh(kn)$ edges and so can be computed in space $\wtilde\bigoh(kn)$.
%%This completes the construction of $G'$.
%
%
%We now argue that $(G,k)$ is a yes-instance of {\sc Edge Bipartization} if and only if $(G',k)$ is a yes-instance. Since $G'$ is a subgraph of $G$, it suffices to argue that if $S$ is a solution for $(G',k)$, then it is also a solution for $(G,k)$. We first notice that $S$ contains all marked edges. This is because an edge $e=(u,v)$ is marked precisely when it is part of $k+1$ odd cycles in $G$ that are pairwise edge-disjoint except in
%$e$. Now, suppose that there is an odd cycle $C$ in $G-S$. Then, it must be the case that $C$ intersects $E(G)\setminus E(G')$. By our construction of $G'$, for every edge $e=(u,v)$ that has not been included in $G'$, it must be the case that there are $k+1$ edge-disjoint odd $u$-$v$ paths in $G'$, at least one of which is disjoint from $S$. For every edge $(u,v)\in E(G)\setminus E(G')$ that appears in the cycle $C$, let $P_{u,v}$ be an odd $u$-$v$ path in $G'-S$. Thus, for every edge  $(u,v)$ in the cycle $C$, we have concluded that there is an odd $u$-$v$ path in $G'-S$. This implies the presence of an odd closed walk in $G'-S$ (simply replace each edge of $C$ contained in $E(G)\setminus E(G')$ with an odd walk between the endpoints) and hence also an odd cycle in $G'-S$, a contradiction.
%
%Therefore, our post-processing algorithm simply invokes, on the instance $(G',k)$, the $\bigoh(3^kk^4(m+n))$-time algorithm for {\sc Edge Bipartization} implied (using the standard reduction) by the $\bigoh(3^kk^3(m+n))$-time $k^{\bigoh(1)}(m+n)$-space algorithm of Kolay et al.~\cite{KolayMRS20} for {\sc OCT}. This completes the proof of the theorem.
%\end{proof}
%
%We remark that the edge variant of {\sc Subset Feedback Vertex Set} is known to be linear-time solvable and given our motivation of designing fixed-parameter semi-streaming algorithms for NP-complete problems, we do not study this problem in this work.


%\red{BISECTION to be added.}

==> preamble-short.tex <==
%Color and Pictures
\usepackage[usenames,svgnames]{xcolor}
\usepackage{graphicx}
\usepackage{tikz}
\usetikzlibrary{decorations.shapes}


%Formatting and Layout
\usepackage{wrapfig}
%\usepackage{fullpage}
\usepackage{xspace}

%Pretty boxes
\usepackage{framed}
\usepackage{boxedminipage}


%Math
\usepackage{amsmath,amssymb}
\usepackage[retainorgcmds]{IEEEtrantools}
\usepackage{pdfpages}
\usepackage{lastpage}
\usepackage[ruled,vlined,linesnumbered]{algorithm2e}
\usepackage{multicol}
\renewcommand{\thefootnote}{\Roman{footnote}}


% Eat up the page numbers: 
%\pagenumbering{gobble}


%Multiple Author Names & Affiliations
\usepackage{authblk}


%Linked References 
%%%\usepackage[pagebackref,linktocpage]{hyperref}
\usepackage{hyperref}

\hypersetup{
    pdfauthor={Neeldhara Misra},     % author
    pdfnewwindow=true,      % links in new window
    colorlinks=true,       % false: boxed links; true: colored links
    linkcolor=SlateBlue,          % color of internal links
    citecolor=FireBrick,        % color of links to bibliography
    filecolor=magenta,      % color of file links
    urlcolor=Emerald           % color of external links
}

%A useful package if you write url addresses:
\usepackage{url}


% Dutch style of paragraph formatting, i.e. no indents. 
%\setlength{\parskip}{1.3ex plus 0.2ex minus 0.2ex}
%\setlength{\parindent}{0pt}





%Macros

\newcommand{\FPT}{\textrm{\textup{FPT}}\xspace}
\newcommand{\WOH}{\textrm{\textup{W[1]-hard}}\xspace}
\newcommand{\WTH}{\textrm{\textup{W[2]-hard}}\xspace}
\newcommand{\NP}{\textrm{\textup{NP}}\xspace}
\newcommand{\NPH}{\textrm{\textup{NP-hard}}\xspace}
\newcommand{\NPC}{\textrm{\textup{NP-complete}}\xspace}

\newcommand{\OO}{{\mathcal O}}
\newcommand{\name}[1]{\textsc{#1}}
\newcommand{\YES}{\textsc{Yes}}
\newcommand{\NO}{\textsc{No}}

\newcommand{\problembox}[4]{
\begin{framed}
{\bf #1} \hfill Parameter: {#3} \\
\begin{tabular}{p{.15\textwidth} p{.8\textwidth}}
% | p{.25\textwidth} p{.7\textwidth} | 
%\hline
\hfill Input: & {#2}\\
%\hfill Parameter: & {#3}\\
\hfill Question: & {#4}\\
%\hline
\end{tabular}
\end{framed}
}



